Evolutionary Defense: Advancing Moving Target Strategies with Bio-Inspired Reinforcement Learning to Secure Misconfigured Software Applications

Improper configurations in software systems often create vulnerabilities, leaving them open to exploitation. Static architectures exacerbate this issue by allowing misconfigurations to persist, providing adversaries with opportunities to exploit them during attacks. To address this challenge, a dynamic proactive defense strategy known as Moving Target Defense (MTD) can be applied. MTD continually changes the attack surface of the system, thwarting potential threats. In the previous research, we developed a proof of concept for a single-player MTD game model called RL-MTD, which utilizes Reinforcement Learning (RL) to generate dynamic secure configurations. While the model exhibited satisfactory performance in generating secure configurations, it grappled with an unoptimized and sparse search space, leading to performance issues. To tackle this obstacle, this paper addresses the search space optimization problem by leveraging two bio-inspired search algorithms: Genetic Algorithm (GA) and Particle Swarm Optimization (PSO). Additionally, we extend our base RL-MTD model by integrating these algorithms, resulting in the creation of PSO-RL andGA-RL. We compare the performance of three models: base RL-MTD, GA-RL, and PSO-RL, across four misconfigured SUTs in terms of generating the most secure configuration. Results show that the optimal search space derived from both GA-RL and PSO-RL significantly enhances the performance of the base RL-MTD model compared to the version without optimized search space. While both GA-RL and PSO-RL demonstrate effective search capabilities, PSO-RL slightly outperforms GA-RL for most SUTs. Overall, both algorithms excel in seeking an optimal search space which in turn improves the performance of the model in generating optimal secure configuration.

==> 3Related_Work.tex <==
\section{Search Space issue in RL-MTD}
In the RL-MTD work, there are two instances where the RL agent has to draw random setting values from the search space range of every parameter $P$ present in a configuration: once during the start state (initial state) of the game when it has generated a random configuration state, other times whenever the action = 1 is chosen and it has to change settings of low score parameters.\newline
As per the STIG website, the permissible default settings are defined for any parameter $P$ belonging to a particular SUT. In our work, as this is a proof-of-concept, we handpicked only those parameters that mostly had integer values and/or 'None' as their settings for ease of computation.
Figure \ref{fig:search} shows how we designed the search space range for the agent to choose from during the RL-MTD operation for any particular SUT. The agent has to learn to eventually choose the permissible secure setting for every parameter P in configuration C from the given search range to ensure  C is close to being secure (goal state). We set the custom space range as follows depending on the data type of setting(P):

\begin{enumerate}
    \item Numeric: $(v-lim, v+lim)$, and
    \item List: choice between $[(0, max(v1,v2,v3..) +lim]$ and  $None$
\end{enumerate}

where $v$ is the default setting value as per the STIG website for any particular SUT, $max(List)$ is the maximum setting value if it is a list type, and $lim$ is an arbitrary integer value. We set $lim = 10$ based on multiple experiments we conducted and this value seemed to give better secure configurations (as we also covered in the Results section).\\
\textbf{Issue:} However, finding the right value of \textit{lim} to define the search space range from where the RL agent picks up random values for parameters can be a time-consuming task and often requires us to play around with a bunch of different values before we can find a good enough candidate. As this search space range is majorly responsible for the performance of RL in terms of generating secure configurations, there is a need to find an optimized search space for RL that is best for agents to generate diverse yet secure configurations. \newline
The solution to this problem is to use search optimization algorithms. In section 5,  we describe how we integrate the bio-inspired search optimization algorithms namely Genetic Algorithm(GA) and Particle Swarm Optimization(PSO) into RL-MTD  and develop Evolutionary RL(E-RL) algorithms for better performance.\newline
We integrate both GA and PSO in our approach because they are widely recognized optimization techniques. PSO operates as a population-based stochastic optimization algorithm, focusing on the collective behavior of swarms \cite {psoadvantage}, while GA functions as a heuristic search-based algorithm, simulating evolutionary processes like crossover and mutation \cite{GA}. Our study aims to compare and assess the performance of these two algorithms to determine which one surpasses the base model in effectiveness.


\begin{figure}[h]
 \begin{center}
      \includegraphics[width=9cm]{images/RL-MTD/search.png}
      \caption{\textbf{Left:} RL-MTD Algo shows the diagrammatic view of all the important functions that use the search space/domain corresponding to a particular SUT. This search range is used by the agent to randomly draw settings from either during the initial config state or when action=1 is chosen.
      \textbf{Right:} shows the search space range for 2 types of parameter settings where the agent has to pick a setting from \{v-lim,v+lim\} if default setting(P) is a single integer value \textit{v} and \textit{lim} is a hyperparameter for a limit of int type; and if default setting(P) could be any value from a list consisting of permissible non-neg integers (v1,v2,v3,...) and/or 'None', it gets to choose either a numerical val from \{0, max( (v1.v2,v3,.)+lim\} or the string value 'None'.
      \textbf{Issue:} How to effectively choose value of \textit{lim} that will optimize the search space range for better performance?}
      \label{fig:search}
      \end{center}
    %\vspace*{-0.2in}
\end{figure}



==> 5MTD_Algorithm_Design.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Bio-inspired RL-MTD Modelling}
\label{sec:methodology}
In this section, we delve into the design of the RL-MTD strategy through the an integrated approach using a Genetic Algorithm with Reinforcement Learning(GA-RL) and Particle Swarm Optimization with RL (PSO-RL). We will elucidate how the components of each algorithm - GA-RL, and PSO-RL - are adapted to our specific context of generating an optimized search space for our RL-MTD algorithm to perform better in generating secure configuration. This is followed by a detailed flowchart presentation, illustrating how these individual strategies are operationalized.
\subsection{Elements Representation for GA-RL, PSO-RL}
Before we dive into the algorithm flow of how MTD is realized using each of these methods, we will first show the element representation used for each bio-inspired algorithm.

\subsubsection{GA-RL} Figure \ref{fig:GA-RL} illustrates how the Genetic Algorithm's (GA) components are represented to be integrated into the RL-MTD(RL) framework. In this model, we have:
\begin{itemize}
    \item \textbf{Gene:} It's an initial random \textit{lim} int value used to define the Lower Limit (LL) and Upper Limit (UL) of a search space corresponding to the datatype of setting(P) as mentioned in section 3. 
    \item \textbf{Chromosome:} It's an individual search space whose range is composed be gene values.
    \item \textbf{Population:} It is a pool made up of different RL-MTD agents each characterized by its search space range. (where each RL agent acts as a chromosome)
\end{itemize}


\begin{figure}[h]
 \centering
      \includegraphics[width=8cm]{images/GA/GAel.png}
      \caption{Genetic Algorithm elements in our GA-RL formulation for MTD.}
      \label{fig:GA-RL}
    %\vspace*{-0.2in}
\end{figure}

The objective is to evolve these different search spaces through the GA with multiple generations. Each RL agent draws from its unique settings search space range to generate random initial configuration states, which are then utilized by the RL algorithm. This algorithm encompasses environment setup, episode generation, and Monte Carlo (MC) prediction functionalities. The initial population consists of a variety of RL agents. Through the iterative processes of Selection, Crossover, and Mutation, this population undergoes evolution across generations. At the culmination of these generations, we identify and select the most effective RL agent from this pool. The selection criteria focus on the agent that achieves the maximum rewards or creates the most secure configurations.

A step-by-step construction of incorporating GA into our RL -MTD is mentioned below. We follow the logic for Selection and Crossover steps similar to the neuroevolution algorithm described in \cite{blog}:
\begin{enumerate}
    \item Treat the \textit{search space} the agent draws from as a chromosome.(We will address the agent's search space as an entire agent for ease of use and consistency throughout the paper)
    \item Agent's parameter,  $lim$ of search range will act as its genes.
    \item The fitness score of secure configurations generated will act as the chromosome’s fitness (i.e. higher the fitness score, the higher the likelihood of survival).
    \item The first iteration starts with $n$ number of agents (search range), all with randomly initialized parameters.
    \item  \textbf{Selection:} By pure chance, some of them will perform better than others. The survival of the fittest option is then implemented by simply excluding the weakest agents from consideration and considering a certain percentage of agents.
    \item \textbf{Crossover:} It is quite risky to swap parameters/genes for the simple reason that it might disturb the best-performing agents' search space range limits. Hence, we rather replicate the selected agents for the next iteration until we reach $n$ agents again for the next iteration.  
    \item \textbf{Mutation:} We modify agents produced during the crossover step, by adding or subtracting a small noise (value) to its parameter(limit). This step ensures we get to explore the neighborhood around the parameters of the best agents in the next iteration.
    \item To secure the best agents from a probable reduction in performance due to the mutation step, we decided to keep the top-performing agent as is (without adding noise).
\end{enumerate} 

\subsubsection{PSO-RL}
%\textcolor{red}{\textbf{NILOOFAR}}
The components in our PSO-RL model as shown in Figure \ref{fig:ps-RL}  are as follows: 
\begin{itemize}
    \item \textbf{Particles / Swarm:} In analogy to Figure \ref{fig:GA-RL}, a particle corresponds to a chromosome in GA, representing a limit \textit{lim}  used to define the search space range. Similarly, akin to the population in GA, a swarm, comprised of a collection of particles, represents a list of limit values defining various search space ranges, thus forming a swarm of distinct RL agents.
    \item \textbf{Particle Position:} Particle represents an individual search space. We denote the particle's position in terms of its fitness. Here fitness is measured by the performance of the RL-MTD model when supplied with that particle.\newline
    $Fitness(particle) = performance(RL-MTD[particle)]$ \newline
    where performance is the agent’s average performance (fitness score) over 60 episodes.
    \item \textbf{Global Best:} In its simplest form, global best refers to the best value of a fitness score among a set of particles. Each particle updates its position at the final stage of the search space exploration, with the best position being identified as the global best.
     \item \textbf{Particle Velocity:} This represents how far a particle position is from the ideal position (fitness). This indicates the moving rates for each particle within the search space. Our study takes advantage of this part to determine the distance between the best particle position and the ideal secure position.

\end{itemize}

\begin{figure}[h]
 \begin{center}
      \includegraphics[width=0.9\linewidth]{images/PSO/psorlel.png}
      \caption{PSO elements in our PSO-RL formulation for MTD.}
      \label{fig:ps-RL}
    %\vspace*{-0.2in}
    \end{center}
\end{figure}

Just like, GA, the goal here is to find the most optimal particle (search space) for our RL-MTD algorithm. The PSO-RL algorithm uses the particle's position, velocity, and global best and is run for 100 generations as per the standard PSO flowchart shown in Figure \ref{fig:PSOflow} to find the most optimal search space for the RL-MTD  model to generate more secure configurations.
\iffalse
Furthermore, the following steps illustrate the procedure we utilize in the experiments:

\begin{enumerate}

\item The initial motivation is to determine the maximum value/position by comparing the preceding value with the current one. This value is considered "Particle Best".
\item When the "Particle Best" reaches its upper-level value, the value aligns with the "Global Best" as well. 
In essence, the peak value attained by the particle aligns with the best global position(Gbest). 
\item Following this, we commence the exploration to identify the optimal value for velocity, where the criterion for optimal is set as the minimum value in our study. 
This minimum value is then substituted for the particle velocity.
\item The computation of particle velocity involves a comparison of both the Optimal Difference and the initial particle velocity values.
The chosen velocity value lies within the range defined by the Optimal Difference and the difference between the ideal fitness value and the particle fitness value corresponding to the limit value. 
\item This distributes as an indicator from an ideal secure configuration.
Notably, a smaller value signifies a more secure search space.

\item The final step involves incorporating social influence, to determine the optimized limit value.
Social influence represents the inertia weight, as well. 
\item The experiment concludes after 100 iterations, with the optimal values for Particle Best, Particle Velocity, and identified Limit value.
    
\end{enumerate}
\fi



\subsection{Bio-inspired MTD Algorithm Design}
In this section, we describe the E-RL algorithms for finding the best-performing agent(search space) to generate a more secure configuration.
\subsubsection{GA-RL}
Algorithm \ref{alg:E-RL} shows how the GA-RL was adapted for finding the best RL agents in generating secure configuration.
\footnote{\raggedright\url{https://github.com/paraschopra/deepneuroevolution/blob/master/openai-gym-cartpole-neuroevolution.ipynb}\par}

\begin{algorithm}[!h]
    \caption{GA\_RL Algorithm to find best RL agents}\label{alg:E-RL}
    \begin{algorithmic}[1]
        \Procedure{perform\_GA}{}
            %\State \textbf{Input:}  $num\_agents$, $num\_generations$, $top\_limit$, $elite\_index = None$
            %\State \textbf{Output:}  $Best Performing Agent$
            \State $num\_agents \gets $ n  \Comment{Initialize n number of agents}
            \State $agents  \gets $ generate\_random\_agents(num\_agents)
            \State $top\_limit \gets k$ \Comment{\# of top agents to consider as parents}
            \For {$gen$ in $range(X)$} \Comment{run evolution until X generations}
                \State $rewards \gets $ run\_agent(agents) \Comment{return rewards of agents}
                \State $selected\_agents \gets $ Select agents of top $k$ rewards \Comment{Selection}
                \State $children\_agents \gets $ Randomly choose $k$-1 agents from $selected\_agents$    \Comment{Crossover}
                \State $mutated\_agents \gets $ Mutate($children\_agents$) \Comment{children agents after Mutation}
                \State $agents \gets mutated\_agents$ \Comment{kill all agents, and replace them with mutated children}
            \EndFor
            \State $Best\_agent \gets$ Select agent from $agents$ with maximum reward
        \EndProcedure
        \State {\bf return} $Best\_agent$
    \end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:E-RL}  follows the pseudo-code mentioned in the previous section. 
\begin{itemize}
    \item With population size set to $n$ ($num\_agents$), we generate agents randomly in the first iteration using the function\newline
    $generate\_random\_agents$ described in Algorithm \ref{alg:gen_agent}
    
    \item We set the maximum number of generations to run the loop to $X$.
    \item The $run\_agent$ function is used in each generation to run all randomly generated agents and get their performance (mean fitness score).(Algorithm \ref{alg:run_agent})
    \item \textit{Selection} : Out of $n$, select only top $k$ as parents ($top\_limit$) where $k<n$.
    
    \item \textit{Crossover}: As mentioned before, we replicate the selected agents instead of swapping parameters. Among top $k$ parent agents,  $k$-1 agents are randomly chosen to make children for the next iteration.
    \item \textit{Mutation}: In the $mutate$ function, we add or subtract a small noise(value) to the parameter if the value of the agent is greater than a random number. (Algorithm \ref{alg:mutate})
    \item After we have child agents as parents, we iterate over the loop again until all generations are done or we find a good performing agent. 
\end{itemize}


\begin{algorithm}[!h]
    \caption{GENERATE AGENTS}\label{alg:gen_agent}
    \begin{algorithmic}[1]
        \Procedure{generate\_random\_agents}{$num\_agents$}
            \State $agents \gets [ ] $ 
            \For {$1$ to $num\_agents$ }
            \State $lim \gets $ Pick \ random \ number from\ range (1, N)  \Comment{N is an integer}
            \State $agents.append(lim)$
            \EndFor
        \EndProcedure
        \State \textbf{return}  $agents$
    \end{algorithmic}
\end{algorithm}

In Algorithm \ref{alg:gen_agent}, function $generate\_random\_agents$ is used to generate $num\_agents$ number of agents . Here the agent represents limit value $lim$ which is an integer value randomly drawn  between 1 and $N$ (hyperparameter). This $lim$  decides the search space range from which the agent picks from.


\begin{algorithm}[!h]
    \caption{RUN AGENT}\label{alg:run_agent}
    \begin{algorithmic}[1]
        \Procedure{run\_agent}{$agents$}
            \State $reward\_agents \gets [ ] $ 
            \For {$ag$ in $agents$ }
            \State $rwrd = run\_RL\_MTD(ag)$ \Comment{Call the $run\_RL\_mc$ func which takes as i/p the agent(i.e lim) }
            \State $reward\_agents.append(rwrd)$
            \EndFor
        \EndProcedure
        \State \textbf{return}  $reward\_agents$
    \end{algorithmic}
\end{algorithm}

In Algorithm \ref{alg:run_agent}, the procedure $run\_agent$ takes a list of agents  $agents$ as input.  For each agent $ag$ in $agents$ list,  $run\_RL\_MTD()$ (Figure 5) is called which takes the agent as input and runs the base RL-MTD model with the new search space ($ag$). The MC prediction (Algorithm \ref{alg:MCP}) method in the RL-MTD model returns the agent's average performance (fitness score) over 60 episodes which is stored in $rwrd$.



\begin{algorithm}[!h]
    \caption{MUTATION}\label{alg:mutate}
    \begin{algorithmic}[1]
        \Procedure{mutate}{$children\_agent$}
            \State $mutate\_agent \gets children\_agent $ 
             \If {$child\_agent$ $>$ $random.random()$}  
                \State $mutate\_agent -= noise$  \Comment{hyperparameter}
            \Else
                \State $mutate\_agent += noise$ 
             \EndIf
        \EndProcedure
        \State \textbf{return}  $mutate\_agent$
    \end{algorithmic}
\end{algorithm}

\subsubsection{PSO-RL}
%\textcolor{red}{\textbf{NILOOFAR}}

In Algorithm \ref{alg:initialpso}, we initialize all the N particles in a swarm with random integers. Each particle's starting position will have the same random integer and the same goes for the particle's velocity. The optimal difference is the hyperparameter we experiment with which indicates the threshold value. This threshold value is to check how far is the particle search space from the optimal one in terms of fitness scores generated from their corresponding RL-MTD agents.

\begin{algorithm}[!h]
    \caption{INITIALIZING N PARTICLES}\label{alg:initialpso}
    \begin{algorithmic}[1]
     \Procedure{initialize}{}
            \State $swarm \gets $ Pick \ N random\ integers \Comment{This is the limit values representing each particle }
            \For {$particle$ in $swarm$}
                \State $particle\_position \gets $ Start \ with \ random \ integer 
                \State $particle\_velocity \gets $  Start \ with \ random \ integer
            \EndFor
            \State $global\_best \gets 0 $ 
            \State $generations \gets 100$ 
            \State $optimal\_difference \gets d$
            \State $ideal\_fitness \gets $ Fitness\ Score\ Ideal\ C \Comment{Its the score of fully secure config}
      \EndProcedure
    \end{algorithmic}
\end{algorithm}

The primary goal of Algorithm \ref{alg:particleposition} is to calculate each particle's current position and update the $gbest$ with the maximum value. The procedure $run\_RL\_MTD()$ (base MTD-RL algorithm)) is called for each value in the swarm. 
The obtained value is then contrasted with the preceding value. The global best receives the new value if the outcomes attained are the highest value.


\begin{algorithm}[!h]
    \caption{PARTICLE POSITION}\label{alg:particleposition}
    \begin{algorithmic}[1]
        \Procedure{maximum\_particle\_position}{}
            \For {$particle$ in $swarm$}
            \State $new\_pp = run\_RL\_MTD(particle)$ \Comment{Call the $run\_RL\_mc$ func }
                \If {$new\_pp$ $>$ $particle\_position[particle]$}  
                    \State $particle\_position[particle] = new\_pp$
                \EndIf
                \State $global\_best = max(new\_pp)$ 
                \EndFor
        \EndProcedure
        \State \textbf{return}  $global\_best$
    \end{algorithmic}
\end{algorithm}

The distance between the ideal fitness and the particle's current position(search space's fitness) is represented by particle velocity. The lesser the distance, the more optimal the particle as it makes the base RL-MTD model generate an almost secure configuration. In Algorithm \ref{alg:particlevelocity}, we are trying to calculate the current distance of the particle (line 3) and we update the particle's old velocity with the current one if the latter is less than the former even though it's still greater than optimal difference (line 4,5). This means it's slowly approaching optimal difference.

\begin{algorithm}[!h]
    \caption{PARTICLE VELOCITY}\label{alg:particlevelocity}
    \begin{algorithmic}[1]
        \Procedure{minimum\_particle\_velocity}{}
            \For {$particle$ in $swarm$}
            \State $new\_pv = ideal\_fitness - particle\_position[particle] $
                \If {$(new\_pv$ $>$ $optimal\_difference)$ and $new\_pv$ $<$ $ particle\_velocity[particle]) $}  
                    \State $particle\_velocity[particle] = new\_pv$
                \EndIf
                \EndFor
        \EndProcedure
         \State \textbf{return}  $new\_pv$
    \end{algorithmic}
\end{algorithm}

In Algorithm \ref{alg:socialinfluence}, $social\_influence$ seeks to improve the particle value in regards to the intermediate best particle via social influence in a particular generation. It attempts to deduct social influence value)or add it depending on whether the current particle is greater or less than the intermediate best particle, thereby trying to converge all the particles to the near-optimal particle.

\begin{algorithm}[!h]
    \caption{SOCIAL INFLUENCE}\label{alg:socialinfluence}
    \begin{algorithmic}[1]
        \Procedure{social\_influence}{} \Comment{particle value learning to be closer to the best one via social influence}
          \For {$particle$ in $swarm$}
             \If {$particle $ $>$ $best\_particle$}  
                \State $particle] -= influence$  \Comment{random float social influence value}
            \Else
                \State $particle] += influence$  
             \EndIf
         \EndFor
        \EndProcedure
    \end{algorithmic}
\end{algorithm}

To determine the optimal $particle$ (search space), Algorithm \ref{alg:generationpso} which is the PSO algorithm is run over 100 generations  
\begin{algorithm}[!h]
    \caption{RUN PSO GENERATIONS}\label{alg:generationpso}
    \begin{algorithmic}[1]
            \For {$gen$ in $generation$ } \Comment{ 100 iteration for finding the best limit\_value}
            \State $maximum\_particle\_position()$
            \State $minimum\_particle\_velocity()$
            \State $social\_influence()$
                \EndFor
            \State \textbf{return}  $particle$
    \end{algorithmic}
\end{algorithm}





\iffalse

\subsection{\textbf{RL Agent evolution with Genetic Algorithm}}

Here, the search space limit is the gene of the corresponding search space of RL agent (chromosome) that is being evolved using the evolutionary algorithm over
generations. Each RL agent uses its corresponding search space to draw random
initial states which is used by the RL algorithm consisting of environment,
generate episode, and MC prediction functionalities. Population is the pool of
different RL agents we initially begin with. Through the process of Selection,
Crossover and Mutation, this pool evolves over generations and we select the single
best-performing RL agent out of the pool after we reach the end of generation.
The best performer is chosen based on the maximum rewards (V) it fetches or secure configurations it generates.
Figure 7.3: Genetic Algorithm elements in our E-RL formulation.
Next section describes the E-RL algorithm for finding the best performing
agent(search space) and generating secure configurations using that range.

Figure \ref{fig:GA-RL} show the elements of GA represented in our RL model. Here, the search space limit is the parameter(gene) of the corresponding search space of RL agent (chromosome) that is being evolved using the evolutionary algorithm over generations. Each RL agent uses its corresponding search space to draw random initial states from which is used by the RL algorithm consisting of environment, generate episode and MC prediction functionalities. Population is the pool of different RL agents we initially begin with. Through the process of Selection, Crossover and Mutation, this pool evolves over generations and we select the single best performing RL agent out of the pool after we reach the end of generation. The best performer is chosen based on the maximum rewards (V) it fetches or secure configurations it generates.

\begin{figure}[h]
 \centering
      \includegraphics[width=10cm]{images/E-RLDiag.png}
      \caption{Genetic Algorithm elements in our E-RL formulation.}
      \label{fig:GA-RL}
    %\vspace*{-0.2in}
\end{figure}


Next section describes the E-RL algorithm for finding the best performing agent(search space) and generating secure configurations using that range.

\section{\textbf{Evolutionary RL for Secure Configuration}}
This section describes the E-RL algorithm withn implementation details and reports results.

\subsection{\textbf{E-RL Algorithm}}

Algorithm \ref{alg:E-RL} shows how the evolutionary-RL was adapted for the finding the the best agents  for the RL in generating secure configuration.\footnote{https://github.com/paraschopra/deepneuroevolution/blob/master/openai-gym-cartpole-neuroevolution.ipynb}

\begin{algorithm}[!h]
    \caption{Evolutionary\_RL Algorithm to generate secure configurations}\label{alg:E-RL}
    \begin{algorithmic}[1]
        \Procedure{perform\_GA}{}
            %\State \textbf{Input:}  $num\_agents$, $num\_generations$, $top\_limit$, $elite\_index = None$
            %\State \textbf{Output:}  $Best Performing Agent$
            \State $num\_agents \gets $ n  \Comment{Initialize n number of agents}
            \State $agents  \gets $ generate\_random\_agents(num\_agents)
            \State $top\_limit \gets k$ \Comment{\# of top agents to consider as parents}
            \For {$gen$ in $range(X)$} \Comment{run evolution until X generations}
                \State $rewards \gets $ run\_agent(agents) \Comment{return rewards of agents}
                \State $selected\_agents \gets $ Select agents of top $k$ rewards \Comment{Selection}
                \State $children\_agents \gets $ Randomly choose $k$-1 agents from $selected\_agents$    \Comment{Crossover}
                \State $mutated\_agents \gets $ Mutate($children\_agents$) \Comment{children agents after Mutation}
                \State $agents \gets mutated\_agents$ \Comment{kill all agents, and replace them with mutated children}
            \EndFor
            \State $Best\_agent \gets$ Select agent from $agents$ with maximum reward
        \EndProcedure
        \State {\bf return} $Best\_agent$
    \end{algorithmic}
\end{algorithm}

Algorithm \ref{alg:E-RL}  follows the pseudo-code mentioned in previous section. 
\begin{itemize}
    \item With population size set to $n$ ($num\_agents$), we generate agents randomly in the first iteration using function $generate\_random\_agents$ described in Algorithm \ref{alg:gen_agent}
    
    \item We set the maximum number of generations to run the loop to $X$.
    \item The $run\_agent$ function is used in each generation to run all randomly generated agents and get their performance (mean fitness score).(Algorithm \ref{alg:run_agent})
    \item \textit{Selection} : Out of $n$, select only top $k$ as parents ($top\_limit$) where $k<n$.
    
    \item \textit{Crossover} : As mentioned before, we replicate the selected agents instead of swapping of parameters. Among top $k$ parent agents,  $k$-1 agents are randomly chosen to make children for the next iteration.
    \item \textit{Mutation} : In $mutate$ function, we add or subtract a small noise(value) to the parameter if the value of agent is greater than a random number. (Algorithm \ref{alg:mutate})
    \item After we have child agents as parents, we iterate over the loop again until all  generations are done or we find a good performing agent. 
\end{itemize}



\begin{algorithm}[!h]
    \caption{GENERATE AGENTS}\label{alg:gen_agent}
    \begin{algorithmic}[1]
        \Procedure{generate\_random\_agents}{$num\_agents$}
            \State $agents \gets [ ] $ 
            \For {$1$ to $num\_agents$ }
            \State $lim \gets $ Pick \ random \ number from\ range (1, N)  \Comment{N is an integer}
            \State $agents.append(lim)$
            \EndFor
        \EndProcedure
        \State \textbf{return}  $agents$
    \end{algorithmic}
\end{algorithm}

In Algorithm \ref{alg:gen_agent}, function $generate\_random\_agents$ is used to generate $num\_agents$ number of agents . Here the agent represents limit value $lim$ which is an integer value randomly drawn  between 1 and $N$ (hyperparameter). This $lim$  decides the search space range from which the agent picks from.


\begin{algorithm}[!h]
    \caption{RUN AGENT}\label{alg:run_agent}
    \begin{algorithmic}[1]
        \Procedure{run\_agent}{$agents$}
            \State $reward\_agents \gets [ ] $ 
            \For {$ag$ in $agents$ }
            \State $rwrd = run\_RL\_mc(ag)$ \Comment{Call the $run\_RL\_mc$ func which takes as i/p the agent(i.e lim) }
            \State $reward\_agents.append(rwrd)$
            \EndFor
        \EndProcedure
        \State \textbf{return}  $reward\_agents$
    \end{algorithmic}
\end{algorithm}

In Algorithm \ref{alg:run_agent}, the procedure $run\_agent$ takes list of agents  $agents$ as input.  For each agent $ag$ in $agents$ list,  $run\_RL\_mc()$ is called which takes the agent as input and runs the environment described for the $mc\_prediction$ algorithm  on the new search space ($ag$). It then returns  the agent's average performance (fitness score) over 60 episodes  which is stored in $rwrd$.



\begin{algorithm}[!h]
    \caption{MUTATION}\label{alg:mutate}
    \begin{algorithmic}[1]
        \Procedure{mutate}{$children\_agent$}
            \State $mutate\_agent \gets children\_agent $ 
             \If {$child\_agent$ $>$ $random.random()$}  
                \State $mutate\_agent -= noise$  \Comment{hyperparameter}
            \Else
                \State $mutate\_agent += noise$ 
             \EndIf
        \EndProcedure
        \State \textbf{return}  $mutate\_agent$
    \end{algorithmic}
\end{algorithm}


\subsection{\textbf{Implementation Details}}
We implemented E-RL algorithm using python 3.6 with libraries numpy and pandas. After much experimentation, we set the following hyperparameters:
\begin{itemize}
    \item number of agents n  = 25
    \item number of top agents k = 5
    \item number of generations X = 100
    \item N = 25
    \item noise = 0.05
\end{itemize}
Fitness function:  To calculate rewards for the agents, we used Monte carlo RL prediction algorithm as the fitness function which we ran with episode count 20 and 60 on that agent and took the average of the scores we got.


\fi








==> 6Experiments_and_Results.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Experiments and Results}
\label{sec:eval}
%a brief introduction of this part
In this section, we elucidate the experimental setup for each algorithm used in implementing MTD: RL-MTD, GA-RL and PSO-RL where we ran each of them on 4 SUT case studies and compared their performance results. We intend to compare each of these models to determine the most effective approach to generating secure configuration using the MTD approach. 

\subsection{Experiment Set Up}
\subsubsection{RL-MTD}
We implemented the algorithm using python 3.6 with libraries numpy and pandas. After much experimentation, we set the following hyperparameters:
\begin{itemize}
    \item lim  = 10 (section 3)
    \item parameter score = HIGH(secure): 800; LOW(not secure): 8 (Section 2.2.3)
    \item Threshold = any value in \texttt{range}:\\
    $(\texttt{max\_score} - \texttt{val}, \texttt{max\_score})$,
    where \texttt{val} is a hyperparameter set to 800, 
    and \texttt{max\_score} is the ideal total fitness score of configuration C  when all parameters are securely set (goal state).  In the action policy, we discourage the agent from selecting the "change" action  if \texttt{fit(C)} falls within this threshold range, as it indicates that all parameters of C are securely set except one. This ensures that the likelihood of the agent choosing action 0 remains high (0.8) in such cases.

    \iffalse
    \item Threshold=  any value in \texttt{range:(max\_score-val,max\_score)}
    where $val$ is a hyperparameter set to 800 and $max\_score$ is the ideal total fitness score of C where all parameters are securely set (goal state).
    In action policy, we discourage the agent to not choosing action change if the fit(C) falls in the threshold fitness range as the range indicates that all parameters of C are securely set except 1. Hence, ensuring the likelihood of the agent taking action 0 is high (0.8) in this case.
    \fi
\end{itemize}


\subsubsection{GA-RL}
We implemented GA-RL algorithm using Python 3.6 with libraries numpy and pandas. After much experimentation, we set the following hyperparameters:
\begin{itemize}
    \item number of agents n  = 25
    \item number of top agents k = 5
    \item number of generations X = 100
    \item N = 25
    \item noise = 0.05
\end{itemize}
\textbf{Fitness function for chromosome:} 
To calculate rewards for different RL agents, we used the complete RL-MTD algorithm as the fitness function. It returns the average of the scores generated by the Monte Carlo (MC) prediction function,  evaluated over episode counts of 20 and 60.


\subsubsection{PSO-RL}
%\textcolor{red}{\textbf{NILOOFAR}}
We implemented the PSO-RL algorithm using Python~3.6, with the libraries \texttt{numpy} and \texttt{pandas}. We set the hyperparameters as follows:
\begin{itemize}
    \item Swarm size  = 30
    \item Particle values (lim): integers = [1....30]
    \item Initial Particle position = 0
    %\item Initial Particle Velocity = 100
    \item Idea Fitness = Maximum fitness score of the most secure configuration based on the selected SUT.
    \item number of generations  = 100
    \item influence = 0.05
\end{itemize}
\iffalse
In Figure \ref{fig:Pso-dia}, the PSO components were implemented in our experimental approach. 
In this context, as mentioned, the "particle" stands as a Limit value as well as the "population" or "swarm" consists of a list of these values.
Our experimental setup was initiated by considering 30 values for the Limit variables, which formed a list ranging from one to 30. 
Subsequently, the preliminary parameters for the particle were set as follows: 
the particle value and the current location or position were formatted to zero, and the particle velocity was set as 100.0.
Furthermore, the stopping criterion was validated on the 100th generation in our study. 
This expresses that we rehearsed our experiment through 100 generations to recognize the optimal particle value.
\fi
% The exploration of our experiment unfolds through the utilization of distinct sets of values for Optimal Difference and Particle velocity. 
% We investigate various scenarios in each case study.
% This methodical approach allows us to comprehensively examine the impact of different parameter combinations on our experiment's outcomes, ensuring an understanding of the optimization process.
\iffalse
\begin{figure}[h]
 \centering
      \includegraphics[width=0.45\textwidth]{images/PSO/Diagramwithicons_301223.png}
      \caption{Particle Swarm Optimization components used in PSO-RL.}
      \label{fig:Pso-dia}
    %\vspace*{-0.2in}
\end{figure}
\fi
%\subsection{Algorithm Design}
Given that configuration C varies across different SUTs due to its diverse parameters, it became evident that employing identical optimal difference and initial particle velocity values to be implemented for all case studies was inappropriate. This is because the values depended on the specific parameters and their quantity within each SUT's configuration. Consequently, we undertook an exploration of various optimal particle and initial particle velocity values to identify the most effective combinations tailored to each SUT. The ultimate goal is to recognize the optimum balance between Particle Velocity and the Optimal Difference. This leads to the attainment of maximum or highly improved results within the PSO-RL framework. 

\iffalse
\begin{figure}[!h]
 \centering
      \includegraphics[width=0.45\textwidth]{images/PSO/Flowchartwithinfo_301223.png}
      \caption{Flowcharts for comparing the PSO model, left: Pso flowchart \cite{PSOflowchart}, right: PSO flowchart used in this study, PP and PV illustrate the Particle Position and Particle Velocity components, respectively.}
      \label{fig:PSOflowchart}
    %\vspace*{-0.2in}
\end{figure}
\fi

We elaborate on the ideal set of hyper-parameters examined for PSO, which comprises the Optimal Difference and Particle Velocity for each case study. 
The ideal set refers to the optimal combination of parameters that led to the most secure and effective results in our experiments.
% These case studies contain Windows 10, McAfee, Microsoft Excel 2016, Microsoft Office 2007, Adobe, and Chrome, respectively. 
% The rationale behind these selections with varied values is to experiment with both lower and higher differences to observe the behavior of the generations.
% Throughout the experiment, diverse combinations of Optimal Difference and Particle Velocity were explored to ascertain the most effective combination.
% To achieve this, our experimental parameters were set within the following ranges:

% \begin{itemize}
% \item Optimal Difference [0, 20, 40, 60, 80, 100]\\
% Particle Velocity [100, 200, 300, 400, 500]
% \item Optimal Difference [100, 120, 140, 160, 180, 200]\\
% Particle Velocity [200, 400, 600, 800, 1000]
% \item Optimal Difference [100, 200, 300, 400, 500]\\
% Particle Velocity [500, 550, 600, 650, 700, 750, 800]
% \item Optimal Difference [500, 1000, 1500, 2000, 2500, 3000]\\
% Particle Velocity [2000, 2500, 3000, 3500, 4000, 4500, 5000]

% \end{itemize}

\iffalse
\begin{table}[h!]
\begin{tabular}{|c|c|}
\hline
 Optimal Difference &  Particle Velocity \\
 \hline
 $[0, 20, 40, 60, 80, 100]$ & $[100, 200, 300, 400, 500]$\\ 
  $[100, 120, 140, 160, 180, 200]$ & $[200, 400, 600, 800, 1000]$\\
 $[100, 200, 300, 400, 500]$ &  $[500, 550, 600, 650, 700, 750, 800]$\\ 
 $[500, 1000, 1500, 2000, 2500, 3000]$ &  $[2000, 2500, 3000, 3500, 4000, 4500, 5000]$\\ 
 \hline
\end{tabular}
\vspace*{0.2in}
\caption{The combination of Optimal Difference and Particle Velocity values to perceive the most secure position}
\label{table:hyperpso}
\end{table}
\fi
% Following the outcomes, a comparison was made with earlier results, including those obtained through Reinforcement Learning and Genetic Algorithms.
Considering these two hyper-parameter values as a tuple (Optimal Difference, Particle Velocity), our best combinations for each case study are as follows:

\begin{itemize}
\item Window 10: (20, 300)
\item McAfee: (300, 500)
\item Microsoft Excel 2016: (160, 200)
\item Microsoft Office 2007: (120, 1000)
% \item Adobe:
% \item Chrome: 
\end{itemize}

% Furthermore, it's important to highlight that among all experimented combinations in the Adobe and Chrome case studies, we consistently attained the maximum level of security in the experiment.
 



\subsection{Results on case studies}
This section demonstrates the performance of all three models: RL-MTD, GA-RL, PSO-RL,  in generating secure configurations and reports the results. Once we get the optimal search space range for both GA-RL and PSO-RL, we run the base RL-MTD with those optimized search spaces and capture their results. We then compare their performance with the base RL-MTD with no optimization.
We selected 4 SUT case studies and the corresponding parameters from the STIG website namely:
 \begin{enumerate}
     \item Windows 10 (59 parameters)
     \item McAfee (14  parameters)
    \item MS Excel (20  parameters)
    \item MS Office (21  parameters)
 \end{enumerate}
These SUTs contain a good number of configuration parameters whose domains are diverse enough. \newline
We executed our developed scripts for varying numbers of episodes and captured the best fitness scores  (i.e., the value of state~$V$, which indicates how secure a given state is).  Figures~\ref{fig:performance} illustrate the trend of fitness scores obtained through the episodes where the x-axis is the episode counts (i.e., between 20-500 episodes); whereas, the y-axis holds the normalized values of fitness scores. More specifically, the normalized fitness score value of 0.0 represents the least secure attained by the agent; whereas, the value 1.0 is the most secure fitness score. The normalization on fitness scores are performed as follows:

\iffalse
\[ 
\begin{aligned}
normalized\_fitness\_score = (fitness\_score - minimum\_fitness\_score)/ \\
(maximum\_fitness\_score - minimum\_fitness\_score) 
\end{aligned}
\]
\fi

\[
normalized(fs) = \frac{fs - min(fs)}{max(fs) - min(fs)}
\]

%where $min(fs)$ for a given fitness score $fs$ is the minimum fitness score of the configuration which is equal to the total sum of multiplying every individual parameter in a configuration with the $LOW$ value. 

where $min(fs)$ for a given fitness score $fs$ is the minimum fitness score of the configuration which is equal to the total sum of the fitness scores for all parameters when they are all set to LOW. Similarly, $min(fs)$ for a given fitness score $fs$ is the maximum fitness score of the configuration which is equal to the total sum of the fitness scores for all parameters when they are all set of HIGH. More specifically,:

\[
min(fs) = \sum_{S_{i} = 1}^{n} LOW\ \ \  ;\ \ \  max(fs) = \sum_{S_{i} = 1}^{n} HIGH 
\]

%it is denoted by   $minimum\_fitness\_score = len(configuration)*LOW$.


%Similarly maximum fitness score is denoted by: $maximum\_fitness\_score = len(configuration)*HIGH $

where $S_{i}$ is the $i$th parameter and $n$ is the total number of parameters. 




%PSO


We now analyze the results for each case study which is also summarized in Table 1.
\subsubsection{Window 10 Case Study}
Upon examining Figure \ref{fig:Hwindows10}, an initial observation reveals that RL-MTD demonstrates the least security performance. However, an instant competition unfolds between GA-RL and PSO-RL (labeled ERL). 
Ultimately, it becomes evident that in this context, PSO-RL outperforms GA-RL, although a slight difference can be depicted. 
Moreover, in this case study, PSO-RL outperformed 17 times in comparison to GA-RL.

\subsubsection{McAfee Case Study}
In this case study, substantial fluctuations are observed across all experiments; however, RL-MTD consistently exhibits inadequate performance compared to the other two methods. Upon initial glance of GA-RL and PSO-RL (labeled ERL) in Figure \ref{fig:Hmsmcoffe}, notable oscillations are evident. Furthermore, both PSO and GA equally performed better than base model for a count of 8 episodes. A distinct pattern emerges in these two methods, while they promote similar performance. 
Specifically, in corresponding episodes, both methods experience periods of insecurity, followed by episodes where performance improves. 
For instance, in episode number 40, the performance of neither algorithm is remarkable, but in the subsequent episode, a notable improvement can be illustrated.

\subsubsection{Microsoft Excel 2016 Case Study}

In this case study, illustrated in Figure \ref{fig:HMSExcel}, RL-MTD and GA-RL (labeled ERL) display predominantly similar and fluctuating behaviors. 
The frequency of episodes where each outperforms the other is comparable.
Although RL-MTD may exhibit better performance in specific episodes, the reverse occurs for GA. 
Despite the oscillations perceived in PSO-RL as a third graph, it consistently surpasses the other two methods in most instances. 
Moving to the episode counts analysis, it becomes evident that the results are outstanding when employing the PSO-RL model in the Microsoft Excel 2016 case study.
In the majority of episodes, PSO-RL demonstrates upper-level performance compared to other methods.

\subsubsection{Microsoft Office 2007 Case Study}


As depicted in Figure \ref{fig:Hmsoffice}, a clear distinction is evident in the performance between RL-MTD and Bio-inspired methods (labeled ERL), including GA-RL and PSO-RL, upon initial glance. 
Although RL-MTD attempts to reach Bio-inspired methods, within one episode, there is a substantial difference in subsequent episodes. 
A slight discrepancy is observed by moving to the GA-RL and PSO-RL methods. 
In most episodes, GA-RL and PSO-RL demonstrate approximate performance. 
However, GA-RL slightly exhibits less security in a few instances. 
It is evident that Bio-inspired methods which are GA-RL and PSO-RL, achieve the highest level of security performance in almost all episodes iteratively. 
This underlines that both GA-RL and PSO-RL attain the higher-rank secure performance.

% \subsubsection{Adobe Case Study}


% In the Adobe case study observed in Figure \ref{fig:Hadobe}, the least secure experiment still belongs to RL upon depicted evidence. 
% This aids that it leads to the lack of GA performance matching. 
% While RL marginally exceeds GA in one episode, the fluctuations occur in subsequent episodes for both experiments. 
% Conversely, PSO reveals the most secure experiment from the outset. 
% This is to say, it achieves maximum security in the initial experiment. 
% It should be noted that, despite fluctuations in RL and GA experiments, PSO consistently reaches the peak level of security from the first step to the entire experiment.

% \subsubsection{Chrome Case Study}

% Upon initial grasp of Figure \ref{fig:Hchrome}, in the Chrome case study, it is evident that the ERL methods express almost similar performance.
% This exhibits that steadily reaches the maximum from the first episodes. 
% The conspicuous observation is the consistently inferior operation of RL among nearly all cases for GA and PSO, comparatively.
% Despite the oscillations in RL, it fails to reach the levels achieved by any of the graphs.

\begin{figure*}[h]
\centering
    \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width=\textwidth]{images/Results/window10-p20v300.png}
      \caption{Windows10}\vspace*{0.1in}
      \label{fig:Hwindows10}
    \end{subfigure}%
    \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width=\textwidth]{images/Results/McAfee-p300v500.png}
      \caption{McAfee}\vspace*{0.1in}
      \label{fig:Hmsmcoffe}
    \end{subfigure}%
    
    \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width=\textwidth]{images/Results/Excel2016-p160-v200.png}
      \caption{MSExcel}\vspace*{0.1in}
      \label{fig:HMSExcel}
    \end{subfigure}%
    \begin{subfigure}[b]{0.45\textwidth}
      \includegraphics[width=\textwidth]{images/Results/office2007-p120v1000.png}
      \caption{MSOffice}
      \label{fig:Hmsoffice}
    \end{subfigure}%
    % \begin{subfigure}[b]{0.33\textwidth}
    %   \includegraphics[width=\textwidth]{images/Results/Adobe-pv-all.png}
    %   \caption{Adobe}
    % \label{fig:Hadobe}
    % \end{subfigure}%
    % \begin{subfigure}[b]{0.33\textwidth}
    %   \includegraphics[width=\textwidth]{images/Results/Chrome-pv-all.png}
    %   \caption{Chrome}
    %  \label{fig:Hchrome}
    % \end{subfigure}
    \vspace*{0.1in}
    \caption{Performance comparison of the 3 models: MTD-RL(labeled RL), GA-RL (ERL-GA), and PSO-RL (ERL-PSO) in generating secure configurations for 4 case studies. The x-axis shows the number of episodes each of the models were trained on and the y-axis shows the normalized fitness each of these models was able to achieve. 1 being the max fitness score: (all parameters securely set) and 0 being the most insecure. From the trend, we see both bio-inspired algorithms outperformed the base RL-MTD model for most of the SUTs reaching almost the most secure config across all episodes. However,  between GA-Rl and PSO-RL, its a close call but as per our analysis in Table 1, PSO-RL was the best performing model by a margin. }
    \label{fig:performance}
    %\vspace{0.5inch}
\end{figure*}

%Table \ref{table:psoresults} summarizes the description of case studies' results.


\begin{table}[h!]
\resizebox{0.47\textwidth}{!}{%
\begin{tabular}{|c|c|c|}
\hline
 Case Studies & Count of episodes (RL, GA-RL, PSO-RL) & Best Algorithm \\
 \hline\hline
 Window 10 & (0, 6, \textbf{17}) & PSO-RL\\ \hline
 McAfee & (0, \textbf{8, 8}) & GA-RL , PSO-RL\\\hline
 MS Excel 2016 &  (0, 2, \textbf{21}) & PSO-RL\\ \hline
 MS Office 2007 &  (0, 0, \textbf{12}) & PSO-RL\\ \hline
 \hline
\end{tabular}
}%
\vspace*{0.2in}
\caption{This table summarizes the results/analysis (Figure \ref{fig:performance}) of the 3 models on each SUT and shows PSO-RL was the clear winner among all 3. We considered 25 number of episodes for each model namely, RL-MTD, GA-RL, and PSO-RL. The values in tuples illustrate the total count of episodes in which each model outperformed the rest two. For instance, for the Windows 10 case study, PSO-RL outperformed others 17 times, while GA-RL did better 6 times. Having said that, in contrast to PSO-RL and GA-RL, base RL-MTD did not achieve better in generating configuration far nay SU. When the cumulative number of episodes is less than 25, the rest of the episodes show equal values between the methods. }
\label{table:psoresults}
\end{table}

\vspace{-1.2em}
% \iffalse

% \subsection{\textbf{Results}}

% %\subsubsection{\textbf{E-RL Results}}

% We ran the E-RL algorithm on the all the 6 platforms  using their best performing agent, to examine the performance of E-RL for generating secure generations over all episode counts. In the next section, we show the E-RL results against the RL results in the same plot for respective SUT's to compare the performance of both the algorithms in generating secure. configurations 

% \subsubsection{\textbf{Performance Comparison: RL vs E-RL}}


% \iffalse
%       \label{fig:Hwindows10}
%       \label{fig:Hadobe}
%       \label{fig:Hchrome}
%       \label{fig:HMSExcel}
%       \label{fig:Hmsoffice}
%       \label{fig:Hmsmcoffe}
%     \label{fig:performance}
% \fi


% Figure \ref{fig:Hwindows10} shows the performance of ERL vs RL algorithm on windows10 case study where it can be evidently seen that the E-RL using {\bf $lim$ = 3.9} (best agent) for search space performed exceedingly well as compared to RL algorithm using $lim$ = 10.0. Here $lim$  value dictates the search space that  the RL algorithm draws values from for parameter settings.

%  For Chrome in \ref{fig:Hchrome}, E-RL managed to generate completely secure configurations for all episodes. The E-RL performed much better than RL for the Adobe (Figure \ref{fig:Hadobe}), McAfee Figure \ref{fig:Hmsmcoffe}) and MSOffice (Figure \ref{fig:Hmsoffice}) platforms in general except the MSExcel platform where the performance was comparable as shown in Figure \ref{fig:HMSExcel} .

% This shows that the genetic algorithm managed to find the optimum search space for generating maximum number of secure configurations. 



% \begin{figure*}[t!]
% \vspace*{-0.02in}
%     \begin{subfigure}{0.33\textwidth}
%       \includegraphics[width=\textwidth]{images/Windowserl.png}
%       \caption{Windows10}
%       \label{fig:Hwindows10}
%     \end{subfigure}%
%     % \begin{subfigure}{0.33\textwidth}
%     %   \includegraphics[width=\textwidth]{images/chromeerl.png}
%     %   \caption{Chrome}
%     %   \label{fig:Hadobe}
%     % \end{subfigure}%
%     % \begin{subfigure}{0.33\textwidth}
%     %   \includegraphics[width=\textwidth]{images/Adobeerl.png}
%     %   \caption{Adobe}
%     %   \label{fig:Hchrome}
%     % \end{subfigure}%
%     \begin{subfigure}{0.33\textwidth}
%       \includegraphics[width=\textwidth]{images/Msofficeerl.png}
%       \caption{MSOffice}
%       \label{fig:HMSExcel}
%     \end{subfigure}%
    
%     \begin{subfigure}{0.33\textwidth}
%       \includegraphics[width=\textwidth]{images/Msexcelerl.png}
%       \caption{MSExcel}
%       \label{fig:Hmsoffice}
%     \end{subfigure}%
%     \begin{subfigure}{0.33\textwidth}
%       \includegraphics[width=\textwidth]{images/Mcafeerl.png}
%       \caption{McAfee}
%       \label{fig:Hmsmcoffe}
%     \end{subfigure}%

%     \caption{Performance comparison of E-RL and RL.}
%     \label{fig:performance}
%     \vspace*{-0.1in}
% \end{figure*}



% \iffalse
% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=10cm]{images/Windowserl.png}
%     \caption{Performance comparison of E-RL and RL on Windows10}
%     \label{fig:winerl}
% \end{figure}


% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=10cm]{images/chromeerl.png}
% %     \caption{Performance comparison of E-RL and RL on Chrome}
% %     \label{fig:cerl}
% % \end{figure}


% % \begin{figure}[!t]
% %     \centering
% %     \includegraphics[width=10cm]{images/Adobeerl.png}
% %     \caption{Performance comparison of E-RL and RL on Adobe}
% %     \label{fig:aderl}
% % \end{figure}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=10cm]{images/Mcafeerl.png}
%     \caption{Performance comparison of E-RL and RL on McAfee}
%     \label{fig:mcerl}
% \end{figure}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=10cm]{images/Msofficeerl.png}
%     \caption{Performance comparison of E-RL and RL on MSOffice}
%     \label{fig:mserl}
% \end{figure}


% \begin{figure}[!t]
%     \centering
%     \includegraphics[width=10cm]{images/Msexcelerl.png}
%     \caption{Performance comparison of E-RL and RL on MSExcel}
%     \label{fig:exerl}
% \end{figure}
% \fi


% \fi




==> 8Conclusion_and_Future_work.tex <==
\section{Conclusion and Future work}
\label{sec:conclusion}
In conclusion, our in-depth research tackles the pervasive challenge of security misconfiguration within software systems—a problem that leaves systems open to exploitation. By integrating bio-inspired algorithms, specifically the Genetic Algorithm (GA) and Particle Swarm Optimization (PSO), into our previously established RL-MTD model, we've advanced the model's proficiency in continuously generating secure and dynamic configurations. Through rigorous comparative analysis, we've ascertained that both the GA-RL and PSO-RL enhancements not only refine the search space for potential configurations but also surpass the original RL-MTD framework in their ability to produce robust configurations against an array of software systems put to the test (SUTs). Noteworthy is the slightly superior performance of PSO-RL in the majority of these scenarios, making it the best-performing model due to a nuanced edge in its search strategy. Our findings represent a significant contribution to the domain of proactive cybersecurity measures. By employing Moving Target Defense (MTD) enriched with machine learning and bio-inspired algorithms, we present an innovative and efficacious strategy to proactively MTD defense strategy from a defender perspective, thereby reinforcing the security posture of software configurations against the dynamic landscape of cyber threats.\newline
For future work, we envision expanding our research to transform the current game model into a more complex and realistic scenario. The next step is to develop a two-player version of the game, where one player is the defender, maintaining secure configurations, while the other acts as an attacker, probing and exploiting vulnerabilities. Additionally, since software applications do not operate in isolation but interact with each other, it is crucial to examine these interactions and how they may impact the Moving Target Defense (MTD) strategy. We also need to study how different configuration parameters influence each other. Ultimately, this research is a stepping stone towards a deeper understanding of how to protect software from misconfiguration threats using MTD, aiming to build a more resilient digital infrastructure.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "main"
%%% End:




==> images/mainflow.tex <==
% \section{Diagrammatic view of Multisketch operations}\label{app:mainflow}  

% A user registers with a user id $\u$ and a vector of biometric templates
% $\mvec=\mvecss{\mlen}$. Multisketch uses two databases $\dbid$ and $\dbmsg$\@,
% where $\dbid$ contains user id $\u$ and the corresponding helper data
% $\sketchval$, and $\dbmsg$ contains the random permutation of the templates
% registered so far. Highlighted are the entries corresponding to a user $\u_4$
% with templates $\mvec_4=\mvec_{41}\ldots\mvec_{4\mlen}$.% and helper
%     % data $\sketchval_4$.
\begin{figure}[t]
  \centering
  \begin{tikzpicture}[
    >=stealth,
    node distance=2cm,
    database/.style={
      cylinder,
      cylinder uses custom fill,
      cylinder body fill=black!25!white,
      cylinder end fill=black!25!white,
      shape border rotate=90,
      aspect=0.25,
      minimum width=2em,
      minimum height=2em,
      draw
    },
    func/.style={
      rectangle,
      fill=red!25!white,
      minimum width=1cm,
      minimum height=1em,
      draw
    },
    cell/.style={
      rectangle,
      draw=black!50!white
    }
    ]
    \node (user) at (0, 0) {User};
    \node[func, right of=user, right=-1.1em, above=3em] (msketch) {$\MS$}; 
    \draw[below of=msketch, dashed, anchor=west] (.85,0.55) rectangle (5.9,-1.2); 
    \node[func, below of=msketch, anchor=east, below=1.95cm,fill=red!10!white,dashed] (mrecover) {$\MRec$};
    % \node[database, right of=user, anchor=south, above=1em, right=2cm] (db1) {$\dbid$};
    \matrix (db1) [right of=user, anchor=south, below=2pt, right=-0.1cm, 
    matrix of math nodes,
    column sep = -\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}}, 
    column 2/.style={nodes={cell}}, 
    anchor=west] {
      \u_1 & \sketchval_1\\
      \u_2 & \sketchval_2\\
      \u_3 & \sketchval_3\\
      |[draw,fill=blue!20]|\u_4 & |[draw,fill=blue!20]|\sketchval_4\\
    };
    \node[left of=db1, anchor=east,right=1.1cm] {$\dbid$};
    \matrix (db2) [right of=db1, left=25pt, matrix of math nodes,
    column sep = 2\pgflinewidth,
    row sep=-\pgflinewidth,
    column 1/.style={nodes={cell}},
    column 2/.style={nodes={cell}}, 
    column 3/.style={nodes={cell}}, 
    column 4/.style={nodes={cell}}, 
    column 5/.style={nodes={cell}}, 
    anchor=west] {
      \mvec_{21} &\mvec_{12} & |[draw,fill=blue!20]|\mvec_{43} &  & \mvec_{3\mlen} \\
      |[draw,fill=blue!20]|\mvec_{41} &\mvec_{32} & \mvec_{33} & |[draw=white]|\ldots & \mvec_{2\mlen} \\
      \mvec_{11} &|[draw,fill=blue!20]|\mvec_{42} & \mvec_{23} &  & \mvec_{1\mlen} \\
      \mvec_{31} &\mvec_{22} & \mvec_{13} & & |[draw,fill=blue!20]|\mvec_{4\mlen} \\
    };
    \node[left of=db2, left=-4pt] {$\dbmsg$};

    % \node[database,right of=db1] (db2) {$\dbmsg$};
    \node[func,below of=db1,anchor=north,above=8pt,left=8pt] (gu) {GetUser};
    \node[func,right of=gu,anchor=east,right=-5pt] (fm) {FindMatches};
    \node[func,below of=db1,anchor=east,below=2em,right=-3pt] (recover) {Recover};

    \draw[->,blue!50,thick] (user.north) |- node[black,near end,above]{$u, \mvec$} node[black,near end,below,font=\small]{register} 
    (msketch.west);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$u, \sketchval$} (db1);
    \draw[->,blue!50,thick] (msketch) -| node[black,near end, left,right]{$\mvec$} (db2);

    \draw[->,blue!50,thick] (user.south) |- ++(1,-0.9) node[black,near end,above]{$u, \mvectilde$} node[black,near end,below,font=\small]{login}   -| node[black,left,near end]{$u$}
    (gu.north);
    \draw[->,blue!50,thick] (user.south) |- ++(0,-0.9)  -- ++(3.1,0) |- node[black,near end, above]{$\mvectilde$}
    (fm.west);
    \draw[->,blue!50,thick] (db1.south) |- node[black,near end,above]{} (gu.east);
    \draw[->,blue!50,thick] (db2.south) |- node[black,near end,above]{} (fm.east);
    \draw[->,blue!50,thick] (gu.south) |- node[black,near end,above]{$\sketchval$} (recover.west);
    \draw[->,blue!50,thick] (fm.south) |- node[black,near end,above]{$\mvec'$} (recover.east);    
    \draw[->,blue!50,line width=2pt] (recover.south) -- node[black,near end,right]{$\mvec$ or $\bot$} ++(0, -0.65);
  \end{tikzpicture}
  % \rcnote{Rough sketch of the flow of the \biosketch.} 
  \caption{Diagram of multisketch as a part of an authentication service. 
  }
  \label{fig:mainflow}
\end{figure}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

